Online Dependent Rounding Schemes for Bipartite Matchings, with Applications

We introduce the abstract problem of rounding an unknown fractional bipartite $b$-matching $\bf{x}$ revealed online (e.g., output by an online fractional algorithm), exposed node-by-node on~one~side. The objective is to maximize the \emph{rounding ratio} of the output matching $M$, which is the minimum over all fractional $b$-matchings $\bf{x}$, and edges $e$, of the ratio $\Pr[e\in M]/x_e$. In analogy with the highly influential offline dependent rounding schemes of Gandhi et al.~(FOCS'02, JACM'06), we refer to such algorithms as \emph{online dependent rounding schemes} (ODRSes). This problem, with additional restrictions on the possible inputs $\bf{x}$, has played a key role in recent developments in online computing. We provide the first generic $b$-matching ODRSes that impose no restrictions on $\bf{x}$. Specifically, we provide ODRSes with rounding ratios of $0.646$ and $0.652$ for $b$-matchings and simple matchings, respectively. This breaks the natural barrier of $1-1/e$, prevalent for online matching problems, and numerous online problems more broadly. Using our ODRSes, we provide a number of algorithms with similar better-than-$(1-1/e)$ ratios for several problems in online edge coloring, stochastic optimization, and more. Our techniques, which have already found applications in several follow-up works (Patel and Wajc SODA'24, Blikstad et al.~SODA'25, Braverman et al.~SODA'25, and Aouad et al.~2024), include periodic use of \emph{offline} contention resolution schemes (in online algorithm design), grouping nodes, and a new scaling method which we call \emph{group discount and individual markup}.

==> stochastic-extension.tex <==
\section{Stochastic Extension}\label{sec:stochastic}



In this section, we generalize our rounding algorithm and its analysis to the following stochastic online bipartite matching problem. 
At each time $t$, an online node arrives, with weight vector $\vec{w}_t\sim \calD_t$, where $\calD_1,\calD_2,\dots$ are a priori known independent distributions. 
A simple example which we focus on for notational simplicity (though our approach generalizes to this problem in full generality) is as follows: each online node $t$ arrives according to a Bernoulli event $A_t\sim \Ber(p_t)$, each each edge $(i,t)$ having some intrinsic value $v_{it}$, but realized weight $w_{it} = v_{it}\cdot A_t$.
This problem (in its full generality) is an online Bayesian selection problem, and a number of algorithms with competitive ratio of $\frac{1}{2}$ are known for it \cite{ezra2020online,dutting2020prophet,feldman2015combinatorial}. By the classic lower bound of Krengel and Sucheston for the single-item prophet inequality problem \cite{krengel1978semiamarts}, the above ratio is best-possible when comparing with the offline optimum algorithm.


In \cite{papadimitriou2021online}, Papadimitriou et al.~initiate the study of this problem in terms of the (polytime) approximability of the optimum \emph{online} algorithm.
Perhaps surprisingly, they show that while for simple cases of the problem (e.g., the single-offline-node problem), the optimum online algorithm is computable using a simple poly-sized dynamic program, in general it is \textsc{pspace}-hard to approximate the optimum online algorithm within some absolute constant $\alpha<1$ (say, $\alpha\approx 0.999999$), and showed that better than $0.5$ approximation can be obtained by polytime online algorithms. This positive results was subsequently improved to $0.526$ implicitly \cite{saberi2021greedy} and to $1-1/e\approx 0.632$ explicitly \cite{braverman2022max}. 
All these results are achieved by rounding the following LP, which can be shown to upper bound the optimum online algorithm's value \cite{papadimitriou2021online,torrico2022dynamic}.
\begin{align}
	\max\quad  & \sum_{i,t} w_{i,t} \cdot x_{i,t} \\
	\textrm{s.t.} \quad & \sum_{t,r} x_{i,t} \leq 1  & \forall i\in [n] \\
	& \sum_{i} x_{i,t} \leq p_{t} & \forall t \\
	& x_{i,t} \leq p_{t} \cdot \left(1-\sum_{t'<t} x_{i,t'}\right) & \forall i,t \label{OPTon-constraint} \\
	& x_{i,t} \geq 0 & \forall i,t.
\end{align}

\begin{lem}
	The optimum of the above LP upper bounds the expected gain of any online algorithm.
\end{lem}

Most of these constraints are evident, and follow from (expected) matching constraints, which appeal also to offline algorithms.
The one constraint which bounds the optimum online algorithm but not the optimum offline one is Constraint \eqref{OPTon-constraint}. This constraint follows from offline node $i$ being matched to $t$ requiring that $t$ arrive, and that $i$ is unmatched before time $t$ --- two events which are independent for online algorithms.

\subsection{Online Rounding for the Stochastic Setting}
As before, to round the LP solution, we would like to guarantee that $\Pr[(i,t)\in \calM \wedge (A_t = 1)] \geq 0.647\cdot x_{i,t}$. 
To do so, at time $t$, if $t$ arrives, then, if we denote by $y_{it} := \sum_{t'<t}x_{i,t}$ the fractional degree of offline node $i\in [n]$ at time $t$ we have node $i$ propose with probability $\frac{x_{i,t,r}(1-\eps+(\delta+\eps)\cdot \mathds{1}[i\not\in L_t])}{p_t\cdot (1-(y_{i,t}\cdot(1-\eps)+(y_{i,t}-\theta)^+\cdot (\delta+\eps)))}$. Changing our notation to let 
$F_{i,t} = 1-\sum_{t'<t}\mathds{1}[(i,t')\in \calM]$ now stand for $i$ not being matched before time $t$, we observe that $$\Pr[F_{it}]\geq \Pr[i \textrm{ proposed prior to time } t] = 1-(y_{i,t}\cdot(1-\eps)+(y_{i,t}-\theta)^+\cdot (\delta+\eps)).$$ 
Similarly, we let $E_{i,t}=1-F_{i,t}$ stand for $i$ having been matched before time $t$.
As for the deterministic setting, we pack nodes $i$ with low fractional degree $y_{i,t}$ into bins of volume $1-\theta$. 
Unlike the previous algorithm, offline nodes propose with the above probability if they are unmatched, rather than only if they did not propose before. Again, these proposals are correlated, in that nodes with low fractional degree at time $t$ are grouped by a bin-packing subroutine, and at most one node per bin proposes to $t$.

The analysis remains essentially unchanged, except for the following lemma, replacing the negative correlation in \Cref{neg-cylinder}.

\begin{lem}\label{stochastic-cylinder-bound}
	For each time $t$ and set of offline nodes $S\subseteq[n]$, we have that
	$$\Pr[E_{S,t}]\leq \prod_{i\in S} U_{i,t},$$
	where $U_{it}:=y_{i,t}\cdot (1-\eps) + (y_{i,t}-\theta)^+\cdot (\delta+\eps)$.
\end{lem}
To prove the above, we need the following claim from  \cite{braverman2022max}. For completeness, we provide a short combinatorial / probabilistic proof of this lemma (see  \cite[Lemma 3.2]{braverman2022max} for an algebraic proof).

\begin{lem}\label{BDM-algebraic-lemma}
    For all $i\in [n]$, let $q_i\in [0,1]$. Then,
    $$\sum_{A\subseteq S} \Pr[E_{A,t},F_{S\setminus A,t}]\cdot \prod_{i\in S\setminus A} q_i = \sum_{A\subseteq S} \Pr[E_{A,t}]\cdot \prod_{i\in A} (1-q_i) \prod_{i\in S\setminus A} q_i.$$
\end{lem}
\begin{proof}
    Consider a probability space where at time $t$ all offline nodes toss a coin with success probability $p_i$, independently.
    The LHS corresponds to all previously free nodes having their coin come up heads.
    The RHS corresponds to the same event, whereby all nodes whose coin came up tails were previously matched. %$(F --> H) \equiv (\neg H --> \neg F)
\end{proof}


\begin{proof}[Proof of \Cref{stochastic-cylinder-bound}]
	The proof is by induction on $t\geq 1$ for all sets $S$. The base case $t=1$, for which $y_{it}\equiv 0$, is trivial. For the inductive step, 
	denote the marginal probability of $i$ proposing to $t$ when $t$ arrives by $$m_{i,t} := \Pr[i\in P_t \wedge (A_t = 1)] = \frac{x_{i,t}\cdot (1-\eps+\mathds{1}[i\in L_t]\cdot (\delta+\eps))}{1-\left(y_{i,t}\cdot (1-\eps) + (y_{i,t}-\theta)^+\cdot (\delta+\eps)\right)}.$$
	%Note that indeed, we propose for any realization $r$ with probability $x$
	\todo{explain this unwieldy expression}
	We note that with this definition, we have that
	\begin{align}\label{U_it-recurrence}
	    U_{i,t+1} \geq U_{it}\cdot (1-m_{it}) + m_{it}.
	\end{align}
	The inductive step follows by noting that at most one of the nodes $i\in S$ may be matched at time $t$, and this requires that any free node in $S$ propose, which happens with probability $m_{i,t}$ (conditioned on any event determined by randomness  up to time $t$ that implies that the node is free), as follows.
	\begin{align*}
		\Pr[E_{S,t+1}] & \leq \sum_{\substack{A\subseteq S \\ |S\setminus A|\leq 1}} \Pr[E_{A,t}, F_{S\setminus A,t}] \cdot \prod_{i\in S\setminus A} m_{i,t}\\
		& = \sum_{\substack{A\subseteq S \\ |S\setminus A|\leq 1}} \Pr[E_{A,t}] \cdot \prod_{i\in A} \left(1-m_{i,t}\right) \prod_{i\in S\setminus A} m_{i,t} & \textrm{Lem \ref{BDM-algebraic-lemma}}\\
		& \leq \sum_{A\subseteq S} \Pr[E_{A,t}] \cdot \prod_{i\in A} \left(1-m_{i,t}\right) \prod_{i\in S\setminus A} m_{i,t} \\
		& \leq \sum_{A\subseteq S} \prod_{i\in A} U_{it} \cdot \prod_{i\in A} \left(1-m_{i,t}\right) \prod_{i\in S\setminus A} m_{i,t} & \textrm{I.H.} \\
		& = \prod_{i\in S}\left(U_i \cdot (1-m_{it}) + m_{it}\right) & \textrm{binomial expansion} \\
		& \leq \prod_{i\in S} U_{i,t+1} & \textrm{Eqn. \eqref{U_it-recurrence}}. &  \qedhere
	\end{align*}
	%The first equality follows from at most one $i\in S$ being matched at time $t$, and the first inequality follows from this event requiring this single node $i$ to propose. 
	%The second equality follows from the following combinatorial argument, where we imagine proposals are made independently (see also \cite[Lemma 3.2]{braverman2022max} for an algebraic proof): for all free nodes to propose (independently) is equivalent to all nodes who did not propose (again, independently) not being free.
	%The second inequality follows from summing over all subsets $A\subseteq S$, including those for which $|S\setminus A|>1$. 
	%The third inequality follows from the inductive hypothesis.
	%The third equality follows from binomial expansion, and the ultimate inequality follows from \Cref{U_it-recurrence}.
\end{proof}

A syntactic generalization of  \Cref{proposal-prob-perturbed} and \Cref{set-proposal-probability} in the deterministic case, whose proof we omit for brevity, implies the following lower bound on the weight of an online node's match.
\begin{lem}
	For each online node $t$, we have that $\Pr[w(\calM(t))\geq w]\geq \sum_{i: w_{i,t}\geq w} 0.647\cdot x_{i,t}$.
\end{lem}

As observed in the proof of the main theorem of \cite{braverman2022max}, by a simple telescoping argument, the above condition suffices to guarantee an approximation of $0.647$.\todo{provide direct proof for completeness}
\begin{lem}
	If for each online node $t$, we have that $\Pr[w(\calM(t))\geq w]\geq \sum_{i: w_{i,t}\geq w} c\cdot x_{i,t}$, then
	$$\E[w(\calM)]\geq c \cdot \sum_{i,t} w_{i,t}\cdot x_{i,t} \geq c\cdot \E[OPT_{on}].$$
\end{lem}

Combining the previous two lemmata, we obtain an improved approximation of the optimum online algorithm's expected gain.

\begin{thm}
	There exists a polytime online stochastic weighted bipartite matching algorithm whose output $\calM$ satisfies 
	$$\E[w(\calM)]\geq 0.647\cdot \E[OPT_{on}].$$
\end{thm}

\section{Two-Sided Vertex Arrivals and Edge Coloring}

\begin{thm}
    There exists an online $1.49\Delta$-edge-coloring algorithm under vertex arrivals in general $n$-node graphs with maximum degree $\Delta=\omega(\log n)$.
\end{thm}
In \emph{multigraphs}, the random bipartition trick of Karloff and Shmoys does not work, but the reduction from edge coloring to rounding fractional matchings assigning value $\frac{1}{\Delta}$ for each edge $e$ (and parallel copies thereof) carries through. We therefore obtain the following.

\begin{thm}
    There exists an online $1.546\Delta$-edge-coloring algorithm under two-sided vertex arrivals in bipartite $n$-node \emph{multigraphs} with maximum degree $\Delta=\omega(\log n)$.
\end{thm}

Finally, we note that edge coloring multigraphs and rounding fractional matchings are in fact equivalent as far as their online approximability. (A similar, less general observation was made in \cite[Appendix F]{cohen2019tight}.) 
Indeed, ... 
\todo{complete}

